Cold-atom sources for the Matter-wave laser Interferometric Gravitation Antenna (MIGA)

The Matter-wave laser Interferometric Gravitation Antenna (MIGA) is an underground instrument using cold-atom interferometry to perform precision measurements of gravity gradients and strains. Following its installation at the low noise underground laboratory LSBB in the South-East of France, it will serve as a prototype for gravitational wave detectors with a horizontal baseline of 150 meters. Three spatially separated cold-atom interferometers will be driven by two common counter-propagating lasers to perform a measurement of the gravity gradient along this baseline. This article presents the cold-atom sources of MIGA, focusing on the design choices, the realization of the systems, the performances and the integration within the MIGA instrument.

==> Biblio.tex <==
@article{Sesana2016,
  doi = {10.1103/physrevlett.116.231102},
  url = {https://doi.org/10.1103/PhysRevLett.116.231102},
  year  = {2016},
  month = {jun},
  publisher = {American Physical Society ({APS})},
  volume = {116},
  number = {23},
  pages = {231102},
  author = {Alberto Sesana},
  title = {Prospects for Multiband Gravitational-Wave Astronomy after {GW}150914},
  journal = {Phys. Rev. Lett.}
}

@Book{Auger2017,
  title         = {An Overview of Gravitational Waves: Theory, Sources and Detection},
  publisher     = {World Scientific Publishing},
  year          = {2017},
  author        = {Auger, G. and Plagnol, E.},
  __markedentry = {[geiger:6]},
  isbn          = {9789813141766},
  url           = {https://books.google.fr/books?id=5dTetAEACAAJ},
}

@article{Aasi2015,
  doi = {10.1088/0264-9381/32/7/074001},
  url = {https://doi.org/10.1088/0264-9381/32/7/074001},
  year  = {2015},
  month = {mar},
  publisher = {{IOP} Publishing},
  volume = {32},
  number = {7},
  pages = {074001},
  author = {J Aasi and others},
  title = {Advanced {LIGO}},
  journal = {Class. Quantum Grav.}
}


@article{shimoda_torsion-bar_2020,
	title = {Torsion-{Bar} {Antenna}: {A} ground-based mid-frequency and low-frequency gravitational wave detector},
	volume = {29},
	url = {https://doi.org/10.1142/S0218271819400030},
	doi = {10.1142/S0218271819400030},
	abstract = {Expanding the observational frequency of gravitational waves is important for the future of astronomy. Torsion-Bar Antenna (TOBA) is a mid-frequency and low-frequency gravitational wave detector using a torsion pendulum. The low resonant frequency of the rotational mode of the torsion pendulum enables ground-based observations. The overview of TOBA, including the past and present status of the prototype development, is summarized in this paper.},
	number = {04},
	journal = {International Journal of Modern Physics D},
	author = {Shimoda, Tomofumi and Takano, Satoru and Ooi, Ching Pin and Aritomi, Naoki and Michimura, Yuta and Ando, Masaki and Shoda, Ayaka},
	year = {2020},
	note = {\_eprint: https://doi.org/10.1142/S0218271819400030},
	pages = {1940003},
}


@article{Acernese2014,
  doi = {10.1088/0264-9381/32/2/024001},
  url = {https://doi.org/10.1088/0264-9381/32/2/024001},
  year  = {2014},
  month = {dec},
  publisher = {{IOP} Publishing},
  volume = {32},
  number = {2},
  pages = {024001},
  author = {F Acernese and others},
  title = {Advanced Virgo: a second-generation interferometric gravitational wave detector},
  journal = {Class. Quantum Grav.}
}

@Article{Akutsu2019,
  author   = {{Akutsu, T. et al}},
  title    = {KAGRA: 2.5 generation interferometric gravitational wave detector},
  journal  = {Nature Astronomy},
  year     = {2019},
  volume   = {3},
  number   = {1},
  pages    = {35--40},
  month    = jan,
  issn     = {2397-3366},
  refid    = {Akutsu2019},
  url      = {https://doi.org/10.1038/s41550-018-0658-y},
}

@misc{ET-design,
  note = {{Einstein Telescope Design Study}, \url{https://www.et-gw.eu/}}
}

@Article{DECIGO2017,
  author        = {{Shuichi Sato et al}},
  title         = {The status of DECIGO},
  journal       = {Journal of Physics: Conference Series},
  year          = {2017},
  volume        = {840},
  pages         = {012010},
  month         = {may},
  __markedentry = {[geiger:]},
  doi           = {10.1088/1742-6596/840/1/012010},
  publisher     = {IOP Publishing},
}

@InProceedings{Lacour2018,
  author        = {{Lacour}, S. and {Nowak}, M. and {Bourget}, P. and {Vincent}, F. and {Kellerer}, A. and {Lapeyr{\`e}re}, V. and {David}, L. and {Le Tiec}, A. and {Straub}, O. and {Woillez}, J.},
  title         = {{SAGE: using CubeSats for gravitational wave detection}},
  booktitle     = {Proceedings of SPIE},
  year          = {2018},
  volume        = {10699},
  series        = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
  pages         = {106992R},
  month         = {Jul},
  adsnote       = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl        = {https://ui.adsabs.harvard.edu/abs/2018SPIE10699E..2RL},
  archiveprefix = {arXiv},
  doi           = {10.1117/12.2313639},
  eid           = {106992R},
  eprint        = {1806.08106},
  keywords      = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena, High Energy Physics - Experiment},
  primaryclass  = {astro-ph.IM},
}

@ARTICLE{Dimopoulos2008,
   author = "S. Dimopoulos and P. Graham and J. Hogan and M. Kasevich and S. Rajendran",
   year = "2008",
   journal = "Phys. Rev. D",
   volume = "78",
   title = "Atomic gravitational wave interferometric sensor",
   pages = "122002",
   url = "https://doi.org/10.1103/PhysRevD.78.122002"
}


@ARTICLE{Chaibi2016,
  title = {Low frequency gravitational-wave detection with ground-based atom interferometer arrays},
  author = {Chaibi, W. and Geiger, R. and Canuel, B. and Bertoldi, A. and Landragin, A. and Bouyer, P.},
  journal = {Phys. Rev. D},
  volume = {93},
  OPTissue = {2},
  pages = {021101},
  numpages = {6},
  year = {2016},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.93.021101},
  url = {https://doi.org/10.1103/PhysRevD.93.021101}
}

@article{Canuel2018,
  doi = {10.1038/s41598-018-32165-z},
  url = {https://doi.org/10.1038/s41598-018-32165-z},
  year  = {2018},
  month = {sep},
  publisher = {Springer Nature America,  Inc},
  volume = {8},
  number = {1},
  pages = {14064},
  author = {B. Canuel and A. Bertoldi and L. Amand and E. {Pozzo di Borgo} and T. Chantrait and C. Danquigny and M. Dovale {\'{A}}lvarez and B. Fang and A. Freise and R. Geiger and J. Gillot and S. Henry and J. Hinderer and D. Holleville and J. Junca and G. Lef{\`{e}}vre and M. Merzougui and N. Mielec and T. Monfret and S. Pelisson and M. Prevedelli and S. Reynaud and I. Riou and Y. Rogister and S. Rosat and E. Cormier and A. Landragin and W. Chaibi and S. Gaffet and P. Bouyer},
  title = {Exploring gravity with the {MIGA} large scale atom interferometer},
  journal = {Sci. Rep.}
}

@article{sabulsky2019fibered,
    title={A fibered laser system for the MIGA large scale atom interferometer},
    author={D. O. Sabulsky and J. Junca and G. Lefèvre and X. Zou and A. Bertoldi and B. Battelier and M. Prevedelli and G. Stern and J. Santoire and Q. Beaufils and R. Geiger and A. Landragin and B. Desruelle and P. Bouyer and B. Canuel},
    year={2020},
    volume = {10},
    number = {1},
    pages = {3268},
    eprint={1911.12209},
    archivePrefix={arXiv},
    primaryClass={physics.atom-ph},
    journal = {Sci. Rep.}
}

@Misc{BertoldiControlSystem,
  year = {2019},
  note = {A. Bertoldi et al, A real-time control system for experiments in amo physics, Submitted to RSI},
}


@Article{Mielec2018,
  author        = {Mielec, N. and Altorio, M. and Sapam, R. and Horville, D. and Holleville, D. and Sidorenkov, L. A. and Landragin, A. and Geiger, R.},
  title         = {Atom interferometry with top-hat laser beams},
  journal       = {Appl. Phys. Lett.},
  year          = {2018},
  volume        = {113},
  number        = {16},
  pages         = {161108},
  month         = oct,
  comment       = {doi: 10.1063/1.5051663},
  doi           = {10.1063/1.5051663},
  OPTissn          = {0003-6951},
  publisher     = {American Institute of Physics},
  url           = {https://doi.org/10.1063/1.5051663},
}

@article{Savoie2018,
  doi = {10.1126/sciadv.aau7948},
  url = {https://doi.org/10.1126/sciadv.aau7948},
  year = {2018},
  month = dec,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {4},
  number = {12},
  pages = {eaau7948},
  author = {D. Savoie and M. Altorio and B. Fang and L. A. Sidorenkov and R. Geiger and A. Landragin},
  title = {Interleaved atom interferometry for high-sensitivity inertial measurements},
  journal = {Sci. Adv.}
}


